The onset of nonpenetrative convection in a suddenly cooled layer of fluid

Conditions for the onset of nonpenetrative convection in a horizontal Boussinesq fluid layer subject to a step change in temperature are studied using propagation theory. A wide range of Prandtl numbers and two different kinematic boundary conditions are considered. It is shown that for high Rayleigh numbers, critical conditions for the onset of convective motion reproduce exactly those for the unsteady Rayleigh-B\'enard instability. Present results extend those of previous research and show a tendency of the rigid-rigid and free-rigid critical curves to converge for low Prandtl numbers. Comparison between present and previously reported results on critical conditions for the onset of instabilities and onset time using different methods yields good agreement on a middle to high Prandtl number range. A ratio of 10 between experimentally measured and theoretically predicted onset times is suggested for stress-free bounded systems.

==> pkg.tex <==

%%% Don't deleete
\makeatletter
\def\ps@pprintTitle{%
  \let\@oddhead\@empty
  \let\@evenhead\@empty
%  \def\@oddfoot{\footnotesize\itshape\ifx\@journal\@empty Preprint\else Preprint, please cite as\ \@journal\fi\hfill}%
\def\@oddfoot{\footnotesize\parbox{\textwidth}{\ifx\@journal\@empty\mbox{}\\*[2\baselineskip]\textit{This is a preprint}\else\mbox{}\\*[2\baselineskip]\fbox{\parbox{\textwidth}{\textit{This is a preprint, with current author affiliations. Please cite using the information below:}\\*[4pt] \@journal}}}\fi\hfill}%
  \let\@evenfoot\@oddfoot}
\makeatother
%%%

\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}

\usepackage{url}      % Load url first
\usepackage{hyperref} % Load hyperref first

%%\usepackage{beton}       % Use Concrete Roman for text
%%\usepackage{concmath}    % Use Concrete Math


\usepackage{psfrag}
\usepackage[final]{showkeys}

\usepackage{psfrag}
\usepackage{graphicx,color}
\usepackage{xspace,enumerate}
\usepackage{amsmath,amssymb}
\usepackage{booktabs}
\usepackage{array}
\usepackage{mathrsfs}
%\usepackage{showkeys}
\usepackage{microtype}
\usepackage{pstricks}
\usepackage{longtable}
\usepackage{lineno}
\usepackage{siunitx}
\usepackage{enumitem}
\usepackage{multirow}

\usepackage{varioref}

\usepackage{rotfloat}
\usepackage{todonotes}

\usepackage{lscape}

\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{longtable}

\synctex=1


%\usepackage{url}
%\usepackage{hyperref}

%\usepackage{libertinus-type1}
%\usepackage{libertine}
%\usepackage{unicode-math}


\usepackage{color}

\hypersetup{
    colorlinks=true,       % Colored links instead of boxes
    linkcolor=blue,        % Color of internal links
    filecolor=magenta,     % Color of file links
    urlcolor=cyan          % Color of external links
}
